Thinking Fast and Slow: Data-Driven Adaptive DeFi Borrow-Lending Protocol

Decentralized finance (DeFi) borrowing and lending platforms are crucial to the decentralized economy, involving two main participants: lenders who provide assets for interest and borrowers who offer collateral exceeding their debt and pay interest. Collateral volatility necessitates over-collateralization to protect lenders and ensure competitive returns. Traditional DeFi platforms use a fixed interest rate curve based on the utilization rate (the fraction of available assets borrowed) and determine over-collateralization offline through simulations to manage risk. This method doesn't adapt well to dynamic market changes, such as price fluctuations and evolving user needs, often resulting in losses for lenders or borrowers. In this paper, we introduce an adaptive, data-driven protocol for DeFi borrowing and lending. Our approach includes a high-frequency controller that dynamically adjusts interest rates to maintain market stability and competitiveness with external markets. Unlike traditional protocols, which rely on user reactions and often adjust slowly, our controller uses a learning-based algorithm to quickly find optimal interest rates, reducing the opportunity cost for users during periods of misalignment with external rates. Additionally, we use a low-frequency planner that analyzes user behavior to set an optimal over-collateralization ratio, balancing risk reduction with profit maximization over the long term. This dual approach is essential for adaptive markets: the short-term component maintains market stability, preventing exploitation, while the long-term planner optimizes market parameters to enhance profitability and reduce risks. We provide theoretical guarantees on the convergence rates and adversarial robustness of the short-term component and the long-term effectiveness of our protocol. Empirical validation confirms our protocol's theoretical benefits.

==> trash/Adversarial-Analysis.tex <==
\newpage
\section{Adversarial Analysis}
\subsection{Price oracle attack}

\begin{definition}
    An attacker with stake $s$ can launch an attack on price oracle during time $t_{\text{begin}}: t_{\text{end}}$ and change the ground truth price process during this time period by $\Delta p$, i.e., if we denote the price random process by $\{\pt\}_t$, the price random process after launching the attack would be $\{\pt'\}_t$ such that $\pt'=\pt, \forall t \in [t_{\text{begin}}: t_{\text{end}}]$
    We will denote such an attack by $\mathtt{ATTACK}(\Delta p, t_{\text{begin}}, t_{\text{end}})$
\end{definition}

How do we quantify the harm that attack $\mathtt{ATTACK}(\Delta p, t_{\text{begin}}, t_{\text{end}})$ causes?

==> trash/Solution.tex <==
\section{Our Protocol Design}
\subsection{Overview}





Our protocol is composed of three components:
(i) The lender agent, identified as \lenderAgent.
(ii) The borrower agent, identified as \borrowerAgent.
(iii) The parameter-selection agent, identified as \parameterAgent.

\lenderAgent and \borrowerAgent are responsible for continuously monitoring the marginal effective interest rates of lenders and borrowers, respectively, in comparison to the external rate. These agents are designed to develop estimations of the expected effective interest rates for lenders and borrowers in the near future, based on the current pool conditions and historical data. We provide more detailed description of these agents later in this section.



The parameter-selection agent (\parameterAgent) leverages the estimates generated by \lenderAgent and \borrowerAgent to determine the pool parameters for the upcoming timeslot. Essentially, the outputs of \lenderAgent and \borrowerAgent act as proxies representing the risk and profit profiles of lenders and borrowers, respectively. These outputs are then fed into \parameterAgent, streamlining its assessment of market conditions. By focusing on a select few key metrics provided by \lenderAgent and \borrowerAgent, rather than dealing with the entire array of pool variables, \parameterAgent is able to operate more efficiently. This approach offers a more structured framework for developing the parameter-selection agent.

For example, an effective \parameterAgent would use the output from \lenderAgent to evaluate the market conditions for lenders. If conditions are unfavorable, it may increase the interest rate (\rt) to compensate lenders or decrease the collateral factor (\colfacN) and \liqthrsh (\liqthrshN) to mitigate future defaults. Similarly, upon receiving the output from \borrowerAgent, if the value is too high, the protocol might adjust the liquidation incentive or the liquidation threshold to make the system more favorable for borrowers.
%
However, it's important to note that modifying the pool parameters typically impacts lenders and borrowers in the opposite direction; And a well-functioning parameter-selection agent must balance these opposing effects to maintain equilibrium in the system.




Our selected strategy for implementing the three agents mentioned above is Reinforcement Learning (RL). However, training these protocol components as RL agents necessitates a simulated environment for interaction. This environment includes (1) a \emph{pool logic} dictating the interactions among pool variables, supplemented by (2) at least one simulated borrower and one simulated lender engaging with the protocol through the pool logic (3) Additionally, we require simulated price and interest rate data, which we can generate using the Brownian motion process mentioned previously.


To meet the first requirement, we simulate a pool logic environment that handles the evolution of pool variables in a deterministic manner; the pool logic's tasks include: (i) applying the interest rate on debt positions, (ii) updating pool variables due to user actions such as joining or leaving the system, (iii) handling liquidation and default events, (iv) enforcing restrictions on lenders' and borrowers' actions based on available assets in the pool, and (v) enforcing collateral factors on borrowers at the time of borrowing, etc.,

Fortunately, we do not need to develop separate simulated lenders or borrowers. For training purposes, we can leverage the lender agent (\lenderAgent) and borrower agent (\borrowerAgent) within the protocol to act as the simulated lenders and borrowers. Essentially, \lenderAgent and \borrowerAgent possess estimations of the future effective interest rate given the pool state, enabling them to make decisions on behalf of lenders and borrowers, respectively. Later in this section, we will delve into how we utilize \lenderAgent and \borrowerAgent both as simulated players and integral parts of the protocol.

It's important to note that training the protocol and the simulated users is an intertwined process. As training progresses, both the protocol and the simulated users improve iteratively. In the subsequent sections, we will provide insights into our approach to the training process and testing. During testing, we can evaluate our protocol with various types of players apart from our simulated players, including human players or those with different degrees of rationality and behavior compared to our simulations.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{image_2024-03-19_13-19-11.png}
    \caption{Protocol overview}
    \label{fig:enter-label}
\end{figure}


\subsection{Lender Agent (\lenderAgent)}


The lender agent is an RL algorithm, that plays the role of a rational lender in the system. It observes the pool state and makes decisions regarding whether to deposit additional funds into the pool or withdraw existing funds. The agent's reward function is the effective interest rate of the lender minus the external risk-free interest rate (with some exceptions that we will cover later).


We employ the $Q$-learning algorithm to train the agent, resulting in the generation of a $Q$-table. This table serves two primary functions: (i) guiding the agent in selecting optimal actions, effectively simulating the role of a lender, and (ii) quantifying the expected marginal value of the system compared to the external market from the lender's perspective across varying pool conditions. Consequently, it offers the necessary insight for \parameterAgent to assess the lender's profit and risk accurately.

\paragraph{State} The agent's state $\state{t}$ at time $t$ is defined as:

\begin{equation}\label{eq:poolstate-def}
    \state{t} = \left\{\lS{\tau}, \bS{\tau}, \cS{\tau}, \uS{\tau}, \rS{\tau}, \pS{\tau}, \colfacN_{\tau}, \liqIncntive_{\tau}, \liqthrshN_{\tau}, \defaultS{\tau}, \rolS{\tau}, \robS{\tau}\right\}_{\tau \in [t-\memory, t]}
\end{equation}

Here, $\memory$ represents the length of the agent's memory, and $\state{t}$ encompasses all the pool variables and history in the last $\memory$ time slots. Throughout this work, we operate under the assumption that the protocol has access to an oracle providing external market interest rates and collateral prices (\pt), therefore past prices and external interest rates are also part of the state.

\paragraph{Action} The action taken at time $t$ is represented by $l_t$ and indicates how much the agent wants to add to or withdraw from its deposit. A negative value for $l_t$ represents a withdrawal, while a positive value indicates lending more assets.
%
In practice, there is a capacity on the agent's available assets, so there is a limit on how much it can add to the system. Moreover, depending on the utilization of the pool, only a fraction of the user's deposit may be withdrawable, and this fraction is determined by the pool logic. 


If the agent successfully executes its action, meaning it doesn't exceed any caps or limits, the change in its deposit in the system is determined by $\lt = \lS{t-1}+l_t$. It's worth noting that in our simulations, we only have one major lender and one major borrower. Consequently, only one lender holds all the deposits in the pool, denoted by $\lt$.





\paragraph{Reward Function} The basic reward function at time $t$ calculates the marginal effective interest rate earned during that timeslot compared to the external interest rate.

\[\text{reward}(\state{t},l_t) = \lt \big(\ut \rt - \poolDefault{t} - \rolt\big) \]

%This reward function effectively accounts for default losses due to collateral price falls and incentivizes the agent to withdraw when the effective interest rate is lower than that of the external market. However, it fails to address a crucial aspect of the system: discouraging high utilization.

%In borrow/lending pools, high utilization is generally undesirable because it restricts users' ability to withdraw funds at any time, effectively binding them to the system. Lenders prefer to avoid situations with very high utilization as it exposes them to increased risks. Conventional borrow/lending protocols address this issue by implementing a steep interest rate curve once the utilization exceeds an optimal threshold. However, this approach is ad-hoc and does not necessarily output the best solution.

%To disincentivize high utilization in our protocol, we introduce an additional term to the reward function. We define an event $\mathcal{W}$ that occurs when a user attempts to withdraw, but the pool logic prevents the withdrawal due to insufficient available funds. In such scenarios, we penalize \lenderAgent proportionally to the intended withdrawal amount, as larger withdrawal attempts signify more significant harm from the inability to withdraw.

%This extra signal alerts the lender that the current state is unfavorable. Consequently, the agent will actively take actions to avoid encountering these unfavorable states in the future. We incorporate this new term into our reward function as follows:

%\[\text{reward}(\state{t},l_t) = \lt \big(\ut \rt - \poolDefault{t} - \indicator{\mathcal{W}}\cdot\left|{l_t}\right| - \rolt\big)\] 


%Without including this additional term, our experiments showed that the utilization often stabilized very close to 1, despite this being an unfavorable situation.

\paragraph{$\mathbf{Q}$-Learning} To train \lenderAgent, we utilize $Q$-learning, where the agent learns a value function denoted as $Q^{\mathcal{L}}(\state{t}, l_t)$. This value function satisfies the Bellman equation:

\begin{equation}
    Q^{\mathcal{L}}(\state{t},l_t) = \text{reward}(\state{t},l_t) + \gamma \cdot\expect_{\state{t+1}} \bigr[ \max_{l_{t+1}} Q^{\mathcal{L}}(\state{t+1},l_{t+1})\bigr]
\end{equation}


The lender agent selects actions by maximizing the $Q$ function at each timeslot:

\[l_t = \max_{\zeta} Q^{\mathcal{L}}(s_t,\zeta) \]

The $Q$ table condenses the lender's risk and profit into a single value, making it easier for planning and subsequent use by the parameter-selection agent. The maintained $Q$ value will be fed to \parameterAgent to offer an estimation of the system's value from the lender's perspective.


\subsection{Borrower Agent (\borrowerAgent)}
The Borrower agent operates similarly to the Lender agent, sharing the same design principles and state space. However, it has a different reward function and action space.

\paragraph{Action}
In each timeslot, the Borrower agent selects two actions: $b_t$ and $c_t$. The first action represents adding or subtracting value from the borrowed amount, while the second action pertains to adjusting the collateral. In practice, we assume a cap on the user's collateral, moreover, the amount a user can borrow is limited by the available assets in the pool. 
If the agent's action does not exceed any cap or limit, the state of the pool will change as follows: $\bt = \bS{t-1} + b_t$, $\ct = \cS{t-1} + c_t$. Again, note that in our simulations we only consider one single borrower therefore the entire debt belongs to one user.



\paragraph{Reward Function} 
The reward function at time $t$ is computed as the external borrowing interest rate subtracted from the protocol's effective interest rate paid during that timeslot. Since in our simulations, there's only one major borrower, $\userLiq{t}{}$ and $\userDefault{t}{}$ represent both the borrower's and the pool's liquidation and default, respectively.



\[\text{reward}(\state{t},l_t) = \bt\bigg(\robt - \big(\rt + \userLiq{t}{} \cdot \liqIncntive - \frac{\userDefault{t}{}}{\bt} \big)\bigg)\]

Similar to the Lender Agent, we employ $Q$-learning and the agent learns a value function $Q^{\mathcal{B}}\big(\state{t},(b_t,c_t)\big)$. This value function is utilized later to train the parameter-selection agent.

\subsection{Parameter-Selection Agent (\parameterAgent)}

The parameter-selection agent utilizes the lender's and borrower's $Q$-functions, along with the pool state from the last $\memory$ timeslots. It then determines the next set of pool parameters $\rt$, $\colfacN_{t}$, $\liqIncntive_{t}$, and $\liqthrshN_{t}$ to maximize a specific reward function, which can be designed in various ways.

The parameter-selection agent doesn't have to be an RL agent, it can be a simpler algorithm that observes predefined patterns in the history and the users' value functions to guide the system toward stability and lower risk. In our simulations, we initially deploy a basic version of \parameterAgent to train \lenderAgent and \borrowerAgent. Once these agents are proficient, we replace the basic parameter-selection agent with an RL agent.

The key idea behind the design of \parameterAgent alongside \lenderAgent and \borrowerAgent is to provide the value functions of the lenders and borrowers to \parameterAgent upfront. This approach streamlines decision-making for \parameterAgent. Because the parameter-selection agent receives the future market conditions directly from the $Q$-functions, it doesn't need to analyze the pool state for each user individually. Therefore, the parameter-selection agent focuses on learning the correct strategies tailored to the varying conditions of lenders and borrowers within the system.

In the following, we provide the specification of \parameterAgent as an RL agent.

\paragraph{State}

The state comprises the pool state in addition to the $Q$-function outputs generated by \lenderAgent and \borrowerAgent. Note that at the start of each timeslot, first \parameterAgent makes a decision and then \lenderAgent and \borrowerAgent make their decisions. Therefore, \parameterAgent does not have access to the state at timeslot $t$ or the $Q$-functions at $t$ when it is making its decision.



\[
\state{t}' = \left\{Q^{\mathcal{L}}(\state{\tau},l_\tau), Q^{\mathcal{B}}\big(\state{\tau},(b_\tau,c_\tau)\big),\lS{\tau}, \bS{\tau}, \cS{\tau}, \uS{\tau}, \rS{\tau}, \pS{\tau}, \colfacN_{\tau}, \liqIncntive_{\tau}, \liqthrshN_{\tau}, \defaultS{\tau}, \rolS{\tau}, \robS{\tau}\right\}_{\tau \in [t-\memory-1, t-1]}
\]

\paragraph{Action}
The action vector is the next timeslot pool parameters i.e.,  $\rS{t}, \colfacN_{t}, \liqIncntive_{t},\liqthrshN_{t}$

\paragraph{Reward Function}

There is significant flexibility in designing the reward function, as it can reflect various objectives behind system design. For instance, one potential reward function could prioritize user engagement, such as $\text{reward}_t = \lt + \bt$, which measures the level of involvement of both lenders and borrowers. The engagement of these two parties serves as an indicator of system stability and competitiveness, given their often conflicting interests. Another option could focus on aligning user value functions closely with those of the external market, emphasizing market competitiveness, expressed as $\text{reward}_t = -|Q^{\mathcal{L}}(\state{t},l_t) - \rolt|-| Q^{\mathcal{B}}\big(\state{t},(b_t,c_t)\big)-\robt|$.


\subsection{Training Process}

To streamline the training process and ensure stability, we adopt a step-by-step approach. Initially, we employ a fixed algorithm for both \parameterAgent and \borrowerAgent while focusing solely on training \lenderAgent. The initial version of \parameterAgent keeps all parameters constant except for \rt, adjusting it based on whether $Q^{\mathcal{L}}(\state{t},l_t) < \rolt$. Meanwhile, the initial \borrowerAgent acts as a myopic agent, borrowing more when $\rt < \robt$ and repaying otherwise.
%

Once \lenderAgent achieves satisfactory stability, we replace \borrowerAgent with an RL agent. And, after training \borrowerAgent well, finally we complete the transition to a fully autonomous and adaptive system by replacing \parameterAgent with an RL agent. 


\subsection{Testing Process}

To conduct tests, we introduce a user simulator proxy that adjusts the outputs of \lenderAgent and \borrowerAgent to simulate diverse user behaviors beyond those encountered during training. For example, the user proxy may occasionally introduce random actions or exhibit biases towards depositing or borrowing rather than withdrawing or repaying. Additionally, we have the flexibility to modify parameters in the price simulators to simulate various price trends.

Devising a systematic approach to create new environment simulators for testing purposes, remains an open problem that we plan to explore in the future.

% \subsection{RL agents ($\mathcal{A}_l, \mathcal{A}_b$)}
% We train two RL agents denoted by $\mathcal{A}_l$ and $\mathcal{A}_b$, to learn the value functions of the lender and borrower, respectively. These value functions respectively denoted by $R_l(s_t)$ and $R_b(s_t)$, quantify the future expected effective interest rate for the lender and borrower, given the pool state $s_t$. The state $s_t$ encompasses all pool variables that are publicly available on the blockchain, such as the lent-out amount, utilization, operational protocol parameters, asset prices, etc.


% To provide a more rigorous definition, let's define the effective interest rate of the lender at any time $t$, denoted by $r_{\text{eff}}^l(t)$. This represents the actual amount received by the lender from the protocol at time $t$, accounting for any defaults that occurred within that specific time slot. Mathematically, it is expressed as:
% \[ r_{\text{eff}}^l(t) = \text{nominal } r_t - \text{default}_t \]

% Here, $r_{\text{eff}}^l(t)$ is crucial in determining the attractiveness of our protocol for lenders.


% Similarly, we can define a concept of effective interest rate for borrowers, denoted by $r_{\text{eff}}^b$, representing the interest rate they are required to pay, added by the liquidation costs and minus the insolvency they generate in that timeslot. In certain markets, such as Compound, where collaterals cannot be lent out, borrowers may also incur a loss due to locking their collateral and the opportunity cost associated with it. Hence:

% \[r_{\text{eff}}^b(t) = \text{nominal } r_t - \text{default}_t + \text{Liquidation cost}_t + \text{Collateral opportunity cost}_t\]


% Based on the definition, $R_l(s_t)$ satisfies the following Bellman equation: (Note that the interest rates are annualized.)
% \begin{equation}
%     R_l(s_t) = \frac{1}{T_{\text{year}}}\cdot r_{\text{eff}}^l(t) + \left(1-\frac{1}{T_{\text{year}}}\right)\cdot E_{s_{t+1}}\left[R_l(s_{t+1})\right]
% \end{equation}


% Similarly, we can write the Bellman equation for $R_b(s_t)$. Using the Bellman equation, $\mathcal{A}_l$ and $\mathcal{A}_b$ learn the value functions.


% \subsection{Parameter-Selection agent ($\mathcal{P}$)}   The primary goal of $\mathcal{P}$ is to leverage $R_{l}(s_t)$ and $R_b(s_t)$ to compare the pool conditions with a risk-free market and adjust the pool parameters to optimize a pre-defined objective function accordingly. The complexity of $\mathcal{P}$ can vary, ranging from a basic fixed-point equation to an advanced RL model capable of selecting the optimal action from a diverse array of action vectors. 

% In the initial version of our simulation, we employ a simple $\mathcal{P}$ that operates as follows: when $R_l(s_t)$ is lower than the risk-free lending interest rate, denoted by $r_l^o$, $\mathcal{P}$ slightly increases the nominal interest rate to compensate the lenders or decreases the collateral factor to prevent further defaults. Conversely, when $R_l(s_t)$ exceeds $r^o_b$, $\mathcal{P}$ reduces the nominal interest rate or increases the reserve factor to prevent overpaying the lenders.
% Similarly, $\mathcal{P}$ can utilize the comparison between $R_b(s_t)$ and $r_b^o$ to adjust parameters that influence borrowers.

% Note that $\mathcal{P}$ should be equipped with an estimation of the external market rates. In our initial implementations, we assume that $\mathcal{P}$ has access to this information through an oracle. However, we can transform this problem itself into a machine-learning problem. By interacting with the users, $\mathcal{P}$ can acquire knowledge about the difference between the external interest rates and $R_l(s_t), R_b(s_t)$, and use this information to update its belief over the external rates.


% In later stages, we can substitute $\mathcal{P}$ with an RL agent that receives $R_l(s_t)$ and $R_b(s_t)$ as input and outputs an optimal set of pool parameters. The reward function for such an RL agent can be tailored to capture the protocol's utility effectively. For example, one might opt to use $|R_l(s_t) - r_l^o|+|R_b(s_t)-r_b^o|$ as the reward function to incentivize competitiveness.


% \subsection{Environment} Our environment consists of simulated lenders, borrowers, a Geometric Brownian motion price simulator, and the pool logic. Importantly, as we train $\mathcal{A}_l$ and $\mathcal{A}_b$, the simulated lenders and borrowers can utilize the trained value function to improve decision-making. As a result, training the protocol and the lender/borrower simulators are interconnected processes. 

% Our simulated lenders/borrowers continue depositing/borrowing at a fixed rate into/from the protocol as long as their value function indicates a respectively higher and lower value compared to the risk-free rates. Otherwise, they withdraw/repay at a fixed rate. However, we have introduced some randomness to the simulated players to (i) prevent the system from converging to a local minimum and (ii) account for irrational or uninformed players.


% \subsection{Training process}  First, we train $R_l(s_t)$ while maintaining $R_b(s_t)$ as a myopic function that solely considers the instantaneous effective interest rate. We utilize a simple fixed-point $\mathcal{P}$ during this phase. Then, we gradually increase the importance of future effective interest rates in training $R_b(s_t)$, while keeping $R_l(s_t)$ unchanged. Note that, simultaneously, our simulated borrowers and lenders also improve as we refine the estimation of $R_l(s_t)$ and $R_b(s_t)$. 

% After adequately training both value functions, we can replace $\mathcal{P}$ with an RL agent and explore different reward functions. Additionally, we can modify certain parameters of the borrower/lender simulator, such as randomness and borrowing/lending rates, to enhance the model's generalization capabilities. 


% \subsection{Testing Process} We can test the protocol's performance by replacing the borrower and lender simulators with different players exhibiting varying degrees of randomness, bias on the value functions, different levels of shortsightedness, and other parameters. We can also change the parameters of the price simulators.

==> trash/protocolObjectives.tex <==
\subsection{Protocol Objectives and Evaluation Metrics}

Our main objective is to design a protocol for a borrowing and lending pool. The protocol aims to achieve the following:
(i) Accurately estimate future market risks for different players based on current market conditions and historical data.
(ii) Utilize this estimation, along with information about risk-free market rates, to dynamically adjust the pool's parameters (\rt, \liqthrshN, \colfacN and \liqIncntive) in real-time and in response to market changes. We now make these points explicit by defining the following metrics of protocol performance.

% \color{red}
% define profit var lar and efficiencies

% define baseline over which the efficiency is defined to produce gains
% \color{black}

\paragraph{Economic security} The protocol should not lose any money over long period of time but in fact in our solution we enforce it in every single 

\paragraph{Competitiveness}The difference between the risk-free rate of lending/borrowing in the external markets compared to the effective interest rates of the protocol tells us the protocol \textit{competitiveness}. The main objective of the interest rate policy is to ensure the protocol tracks these external rates as closely as possible.


\paragraph{Profit}


We define the profit of a borrowing position from a lender's perspective as the sum total of all cash flows into the lender's account. This includes interest rate payments and any assets lost to insolvencies.

\paragraph{Value-At-Risk (VaR)} 

VaR is a statistical measure that estimates the minimum potential profit of lending position after time \( T \), given a certain confidence level \( \alpha \) (e.g., 95\% or 99\%). Mathematically, VaR can be defined as:

\[
\text{VaR}_\alpha (T) = - \inf \left\{ x \in \mathbb{R} : P(X < x) \leq 1 - \alpha \right\}
\]

where \( X \) is the profit of the borrow position over the time period \( T \), \( \alpha \) is the confidence level (e.g., 0.95 for 95\% confidence), \( P(X > x) \) is the probability that the profit \( X \) is below the value \( x \).


\paragraph{Liquidations-At-Risk (LaR)} 
LaR is a statistical measure that estimates the maximum liquidation of lending position after time \( T \), given a certain confidence level \( \alpha \) (e.g., 95\% or 99\%). Mathematically, LaR can be defined as:

\[
\text{LaR}_\alpha (T) = - \inf \left\{ x \in \mathbb{R} : P(L > x) \leq 1 - \alpha \right\}
\]

where \( L \) is the total amount of liquidations over time \( T \), \( \alpha \) is the confidence level (e.g., 0.95 for 95\% confidence), \( P(L > x) \) is the probability that the liquidations \( L \) exceeds the value \( x \).



\paragraph{Baseline Protocol}
The baseline protocol follows fixed interest rate curves and selects the one which aligns with the equilibrium equation when considering the current expected default rate, mimicking the approach of established DeFi lending protocols. The interest rate is given by
\begin{align}
    r_{t+1} = \mathcal{I}_{\{U_t \leq U^*\}} b_1 U_t + \mathcal{I}_{\{U_t > U^*\}} (b_1 U^* + b_2 (U_t - U^*))
\end{align}
where $\mathcal{I}_{\{.\}}$ is an indicator function, and $b_1 < b_2$ are fixed slope parameters to encourage borrowers/lenders to stay at the desired utilization.

\paragraph{Risk Efficiency}
Finally, we use the notion of risk efficiency to compare our protocols to a baseline. We say that protocol 1 is more \textit{risk-efficient} than protocol 2 if protocol 1 has a larger profit for the same or less VaR value. We aim to develop a lending protocol that is more risk-efficient than the baseline. The main driver behind setting $LT$ should be to make the protocol more risk-efficient.










==> trash/stochasticModel.tex <==
\section{game Theoretic Model}


\begin{algorithm}[H]
\SetAlgoLined
\caption{Pool variables interaction in the 3 players game}
%\KwIn{Parameters $i$, $\sigma$}
%\KwOut{Values for $\lt(i)$, $\bt(i)$, $\ct(i)$, and $\params{t+1}$}
\textbf{Initialization:}\begin{itemize}
    
    \item Initialize $\rS{0}$.
    \item Sample $\pS{0}$
    \item Initialize $\lS{0}^+$, $\bS{0}^+$ and $\cS{0}^+$ such that $\frac{\bS{0}^+ }{\cS{0}^+ \pS{0}}<\colfacN$.
\end{itemize}
\medskip



\While{$t \leq T$}{
    \begin{itemize}
        \item Sample $\pS{t+1}$
        \item \textbf{Default calculation:} Calculate $\poolDefault{t}=\max\{0,\bt-\ct\cdot\pS{t+1}\}$
        \item \textbf{Default application:} Initialize $\bS{t+1}^{-} = \bt^+ - \poolDefault{t}$  and $\lS{t+1}^-=\lt^+ - \poolDefault{t} $, $\cS{t+1}^-=\ct^+ $.
        \item \textbf{Liquidation calculation:} If $\frac{\bS{t+1}^-}{\cS{t+1}^- \cdot \pS{t+1}}> \liqthrshN$, set  $\,\userLiq{t}{}=\frac{\bS{t+1}^--\liqthrshN \cdot \cS{t+1}^- \cdot \pS{t+1}}{1-\liqthrshN (1+\liqIncntive)}\,$  otherwise set $\userLiq{t}{} = 0$.
        \item \textbf{Liquidation application:} If $\userLiq{t}{}>0$ then set $\bS{t+1}^- = \bS{t+1}^- - \userLiq{t}{}$ and $\cS{t+1}^- = \cS{t+1}^- - \frac{\userLiq{t}{}\cdot (1+\liqIncntive)}{\pS{t+1}} $.
        \item \textbf{Interest rate application:} $\bS{t+1}^- = \bS{t+1}^- \cdot (1+\rt)\quad$, $\lS{t+1}^- = \lS{t+1}^- + \rt \cdot \bS{t+1}^-$.
        \item \textbf{Protocol action:} Protocol selects $\rS{t+1}$.
        \item \textbf{Lender action selection:} The lender picks $\Delta \lS{t+1}$,
        \item \textbf{Lender action process:} If $\Delta \lS{t+1}>0$, pool immediately applies $\lS{t+1}^+ = \lS{t+1}^-+\Delta \lS{t+1}$, but if  $\Delta \lS{t+1}<0$, this gets applies only if $\left|\Delta \lS{t+1}\right| < \lS{t+1}^- - \bS{t+1}^-$. 
        \item \textbf{Borrower action selection:} The lender picks $\Delta \bS{t+1}$ and $\Delta \cS{t+1}$.
        \item \textbf{Borrower action process:} The pool logic assesses if $\frac{\bS{t+1}^-+\Delta \bS{t+1}}{\cS{t+1}^-+\Delta \cS{t+1}} < \colfacN$, if it was not the case, the borrower's action gets ignored and the algorithm goes to the next line. Otherwise, the pool verifies that in the case of borrow i.e., $\Delta \bS{t+1} >0$, $\Delta \bS{t+1} $  is less than the available asset in the pool $\lS{t+1}^- - \bS{t+1}^-$. If this was the case or if the borrower's action is repaying i.e., $\Delta \bS{t+1} <0$, then the pool applies $\bS{t+1}^+=\bS{t+1}^-+\Delta \bS{t+1}$,  $\cS{t+1}^+=\cS{t+1}^-+\Delta \cS{t+1}$ otherwise the pool ignores the borrower's action.
        \item $t \gets t+1$
        
    \end{itemize}
    
}


\end{algorithm}


\paragraph{Lender's effective interest rate} The balance of the lender at the beginning of the timeslot $[t,t+1]$ is $\lt^+$ and at the end of the timeslot is $\lS{t+1}^- = (\lt^+-\bt^++\userLiq{t}{}) + (1+\rt) \cdot \big(\bt^+ - \poolDefault{t}-\userLiq{t}{}\big)$, his change of balance is: 

\[\lS{t+1}^- - \lt^+ = -\poolDefault{t} + \rt \cdot \big(\bt^+ - \poolDefault{t}-\userLiq{t}{}\big) \approx -\poolDefault{t} + \rt \ut \lt\].
\[\text{payoff}_t^l = \bigg( \rt \cdot \big(\bt^+ - \poolDefault{t}-\userLiq{t}{}\big) - \poolDefault{t}\bigg) - \rolS{}\lt^+ \]

% His effective interest rate during this timeslot is: 
% \[ r^l_{\text{eff}} = \frac{ -\poolDefault{t} + \rt \cdot \big(\bt^+ - \poolDefault{t}-\userLiq{t}{}\big)}{\lt^+} \]



\paragraph{Borrower's effective interest rate} The debt of the borrower at the beginning of the timeslot $t$ is $\bt^+$, and at the end of the timeslot it is $\bS{t+1}^- = \big(\bt^+ - \poolDefault{t}-\userLiq{t}{}\big) \cdot (1+\rt)$, Moreover he pays $\userLiq{t}{}\cdot (1+\liqIncntive) $ as a result of the liquidation. What the borrower pays during this timeslot is: 
\begin{align*}
\text{Added liability and costs} &=\bS{t+1}^-  - \bt^+ + \userLiq{t}{}\cdot (1+\liqIncntive) \\&= \bt^+ \rt - (\poolDefault{t}+\userLiq{t}{}) \cdot (1+\rt) + \userLiq{t}{} \cdot (1+\liqIncntive) \\
&= \bt^+ \rt - \poolDefault{t} \cdot (1+\rt) + \userLiq{t}{} \bigr(\liqIncntive - \rt\bigr)\\&\approx
\bt^+ \rt  - \poolDefault{t} + \userLiq{t}{}\cdot\liqIncntive
\end{align*}

\[\text{payoff}_t^b = \bt^+ \robt - \bigg(\bt^+ \rt - \poolDefault{t} \cdot (1+\rt) + \userLiq{t}{} \bigr(\liqIncntive - \rt\bigr)\bigg)\]

Without considering the liquidation incentive term:
\begin{align}
    \text{payoff}_t^b  + \text{payoff}_t^l &= \bt^+ \robt - \lt^+ \rolt \\&= \underbrace{\bt^- \robt - \lt^- \rolt}_{\text{part of the state}} + \underbrace{\Delta \bt \robt - \Delta \lt \rolt}_{\text{negligible}}
\end{align}

Therefore the game is zero-sum as long as $\Delta\lt \ll \lt$ and $\Delta \bt \ll \bt$.





\newpage
\begin{algorithm}[H]
\SetAlgoLined
\caption{Interaction of rational users and protocol in a Borrow/Lending pool}
%\KwIn{Parameters $i$, $\sigma$}
%\KwOut{Values for $\lt(i)$, $\bt(i)$, $\ct(i)$, and $\params{t+1}$}
\textbf{Initialization:}\begin{itemize}
    \item Set $t = 1$
    \item Define $\params{\tau} \coloneqq [\rS{\tau}, \liqIncntive_{\tau} , \liqthrshN_{\tau}, \colfacN_{\tau}]$, and sample $\params{1}$ randomly.
\end{itemize}
\medskip



\textbf{\color{blue}{Lenders}}



\begin{align*}
    \lt(i) =  &\arg\max_{l \in \mathbb{R}^+}\Bigg(\sum_{\tau = t}^{T} \mathbb{E}\biggr[\lS{\tau}(i)\big(\uS{\tau} \rS{\tau} - \poolDefault{\tau} - \rolS\big)\mid \lt(i)=l, \params{t},\rolt, \robt,\pt\biggr]\Bigg)\\
    &\text{subject to} \quad  \lS{t-1} - l \leq   (1-\uS{t-1})\lS{t-1}\quad \text{and} \quad l < \text{cap}_i 
\end{align*}

%\tcc{The lender is constrained by the available assets, meaning they cannot withdraw more than what is currently held, and by their capacity, indicating they cannot deposit more than their maximum limit allows.}


\textbf{\color{blue}{Borrowers}}
\begin{align*}
    \bt(i) =  &\arg\min_{b \in \mathbb{R}^+} \sum_{\tau=t}^{T} \mathbb{E}\biggr[\bS{\tau}(i) \Big(\rS{\tau} + \userLiq{\tau}{i} \cdot \liqIncntive_{\tau} - \frac{\userDefault{\tau}{i}}{\bS{\tau}(i)} - \robS\Big)\mid \bt(i) = b, \params{t}, \robt,\rolt,\pt\biggr]\\
    &\text{subject to} \quad  b - \bS{t-1} \leq   (1-\uS{t-1})\lS{t-1}\;
\end{align*}
\begin{align*}
    \bt(i) =  &\arg\min_{b \in \mathbb{R}^+} \sum_{\tau=t}^{T} \mathbb{E}\biggr[\bS{\tau}(i) \Big(\rS{\tau} - \robS\Big)\mid \bt(i) = b, \params{t}, \robt,\rolt,\pt\biggr]\\
    &\text{subject to} \quad  b - \bS{t-1} \leq   (1-\uS{t-1})\lS{t-1}\;
\end{align*}
\begin{align*}
    \ct(i) =  \max\{\cS{t-1}, \frac{\bt(i)}{\pt\colfacN_t}\}\;
\end{align*}

\textbf{\color{blue}{Protocol}}
\begin{align*}
    \params{t+1} =  &\arg\min_{\mathbf{p} \in [0,1]^4}\Bigg(\sum_{\tau = t+1}^{T} \mathbb{E}\biggr[\big(|\uS{\tau} \rS{\tau} - \poolDefault{\tau} - \rolS|\big)\mid \params{t+1} = \mathbf{p}\biggr]\Bigg)\\
    %&\text{subject to} \quad \text{Var}\Big(\sum_{\tau = t+1}^{T} \lS{\tau}\big(\uS{\tau} \rS{\tau} - \poolDefault{\tau} - \rolS\big)\mid \params{t+1} = \mathbf{p}, \lt, \bt(i), \ct(i), \pt, \rolt, \robt\Big) < \sigma\;
\end{align*}
\textbf{\color{blue}{Environment}}
\begin{itemize}
    \item Sample $\pS{t+1}$ according to the asset price model.
    
\end{itemize}

\medskip
\textbf{\color{blue}{Pool logic}}
\begin{itemize}
    \item Calculate $\userDefault{t}{i}, \userLiq{t}{i}, \forall i \in \users$ according to equations \ref{eq:userDefault}, \ref{eq:userLiq}.
    \item Calculate $\poolDefault{t}$ according to equation \ref{eq:poolDefault}
    
    \item Apply the nominal interest rate of the borrowers for the last timelost i.e., $\bt(i) = \bt(i)  \cdot (1 + \rt ),\; \forall i \in \users$

    \item Apply the effective interest rate of the lenders for the last timelost i.e., $\lt(i) = \lt(i)  \cdot (1 + \ut \rt - \poolDefault{t} ),\; \forall i \in \users$

    
\end{itemize}


\end{algorithm}
\newpage
